Detailed optical spectroscopy of the B[e] star MWC 17

Based on the data of multiple high-resolution R=60 000 observations obtained at the 6-meter telescope BTA in combination with the NES spectrograph, we studied the features of the optical spectrum of the star MWC 17 with the B[e] phenomenon. In the wavelength interval 4050-6750 A we identified numerous permitted and forbidden emissions, interstellar NaI lines, and diffuse interstellar bands (DIBs). Radial velocities were estimated from lines of various origin. As the systemic velocity, Vsys, the velocity from the forbidden emissions can be accepted: Vr=-47 km/s (relative to the local standard Vlsr=-42 km/s). Comparison of the obtained data with the ealier measurements allows us to conclude on the absence of considerable variability of spectral details.

==> longtab.tex <==

\begin{longtable}{l llc@{\quad} @{\quad}l @{\quad}l @{\quad}l@{\quad}}
\caption{Отождествление линий, их остаточные интенсивности
              и лучевые скорости ${\rm V_r }$\,, км/сек в спектре
	      Cyg\,OB2 - ${\rm \No}$\,12. В скобках указан номер мультиплета
	      }      
\\ \hline
\endfirsthead
\hline
\multicolumn{6}{l}{Табл.\,1, продолжение} \\ \hline
\endhead
\hline
\multicolumn{6}{r}{продолжение на след. странице} \\ \hline
\endfoot
\hline
\endlastfoot
\hline
 Е & & ${\rm \lambda_{lab}}$ &  W$_{\lambda}$, \AA & r  & ${\rm V_r }$  \\
\hline

\hline
\end{longtable}	       			     
\label{lines}

